Shoal++: High Throughput DAG BFT Can Be Fast!

Today's practical partially synchronous Byzantine Fault Tolerant (BFT) consensus protocols trade off low latency and high throughput. On the one end, traditional BFT protocols such as PBFT and its derivatives optimize for latency. They require, in fault-free executions, only 3 message exchanges to commit, the optimum for BFT consensus. However, this class of protocols typically relies on a single leader, hampering throughput scalability. On the other end, a new class of so-called DAG-BFT protocols demonstrates how to achieve highly scalable throughput by separating data dissemination from consensus, and using every replica as proposer. Unfortunately, existing DAG-BFT protocols pay a steep latency premium, requiring on average 10.5 message exchanges to commit a transactions. This work aims to soften this tension and proposes Shoal++, a novel DAG-based BFT consensus system that offers the throughput of DAGs while reducing commit latency to an average of 4.5 message exchanges. Our empirical findings are encouraging, showing that Shoal++ achieves throughput comparable to state-of-the-art DAG BFT solutions while reducing latency by up to 60%.

==> Makefile <==
.PHONY: FORCE lenny all clean distclean

FILE=main

all: $(FILE).pdf

%.pdf: %.tex FORCE
	latexmk -pdf -f -e '$$pdflatex=q/pdflatex %O %S/' $<

fast:
	pdflatex $(FILE)


clean:
	for ext in aux log toc lof lot lol dlog bbl \
		nav snm fls vrb blg out tpt fdb_latexmk; \
	do \
		$(RM) $(FILE).$$ext ; \
	done
	$(RM) *.aux *.bak *~

distclean: clean
	$(RM) $(FILE).pdf
	$(RM) $(FILE).ps
	$(RM) $(FILE).dvi
	$(RM) *.d

read: all
	open $(FILE).pdf


==> code/tmp.tex <==
\begin{algorithm}[H]
\caption{Eventually synchronous \sys: algorithm for party $p_i$.}
\begin{algorithmic}[1]
\alglinenoPop{counter}
\small

        \Statex \textbf{Local variables:}
      
        \StateX $\mathsf{orderedVertices} \gets \{\}$
        \StateX $\mathsf{lastOrderedRound} \gets 0$
        \StateX $\mathsf{orderedAnchorsStack} \gets $ initialize empty stack
    
       \Statex
       
    
        \Procedure{\textsc{TryCommitting}}{$\mathsf{v}$}
         \If{$\mathsf{v}.\textit{round} \text{ mod }2 = 1$  or $\mathsf{v}.\textit{round} = 0$}
            \State return 
        \EndIf    
    
        \State $\mathsf{anchor} \gets$ \textsc{getAnchor($\mathsf{v}.\textit{round-2}$)}
        \State $\mathsf{votes} \gets \mathsf{v}.\textit{edges}$
        \If{$|\{ \mathsf{v'} \in \mathsf{votes}: \textsc{path}(\mathsf{v'},\mathsf{anchor})\}|
        \geq f+1$}
        
        \State \textsc{orderAnchors($\mathsf{anchor}$)}
        
        \EndIf 
        
        
    \EndProcedure
       
     \StateX
    
    
    
    \Procedure{\textsc{orderAnchors}}{$\mathsf{v}$}
        \State $\mathsf{anchor} \gets \mathsf{v}$
        \State $\mathsf{orderedAnchorsStack}.\textit{push}(\mathsf{anchor})$
        \State $\mathsf{r} \gets \mathsf{anchor}.\textit{round} -2$
        \While{$\mathsf{r} > \mathsf{lastOrderedRound}$}
        \State $\mathsf{prevAnchor} \gets \textsc{getAnchor}(\mathsf{r})$
            
            \If{$\textsc{path}(\mathsf{anchor}, \mathsf{prevAnchor})$}
            \State $\mathsf{orderedAnchorsStack}.\textit{push}(\mathsf{prevAnchor})$
            \State $\mathsf{anchor} \gets \mathsf{prevAnchor}$ 
            
        \EndIf
        
        \State $\mathsf{r} \gets \mathsf{r} -2$
        \EndWhile
        
        \State $\mathsf{lastOrderedRound} \gets \mathsf{v}.\textit{round}$
        \State $\textsc{orderHistory()}$
        
    \EndProcedure
    
    \Statex
    
    \Procedure{\textsc{orderHistory()}}{}
        \While{$\neg \mathsf{orderedAnchorsStack}.\textit{isEmpty}()$} 
        \State $\mathsf{anchor} \gets \mathsf{orderedAnchorsStack}.\textit{pop}()$ 
          \State $\mathsf{verticesToOrder} \gets \{\mathsf{v} \in \bigcup_{\mathsf{r} > 0}
        \mathsf{DAG_i[r]} \mid \textsc{path}(\mathsf{anchor},\mathsf{v}) \wedge \mathsf{v} \not\in $
       $\mathsf{orderedVertices}\}$
          \For{$\textbf{every} ~\mathsf{v} \in \mathsf{verticesToOrder}$ in some deterministic order}
              \State \textbf{order} $\mathsf{v}$
              \State $\mathsf{orderedVertices} \gets \mathsf{orderedVertices} \cup \{\mathsf{v}\}$
          \EndFor
        \EndWhile
        \EndProcedure  
    
    
\end{algorithmic}
\label{alg:ESBullshark}
\end{algorithm}


==> sections/1-introduction.tex <==
\section{Introduction (Old)} 
\label{sec:introduction}
\fs{don't like "Shoal++", just the name itself sounds very incremental PLUS it may be violation of anonymity. If anything call it ShoalNG, but I think giving a fully self-standing name is strictly better. (It's also confusing to have both Mako and Shoal++ for different things.} %Mako: Unshackling DAG BFT Latency

\fs{making notes (commented out) for some re-write.}
\fs{Question: Is talking about Quorum store necessary at all?}


After over 40 years of research, Byzantine fault-tolerant (BFT) systems have finally transitioned from being mere academic curiosities to practical, widely deployed solutions.
Numerous blockchain companies~\cite{aptos, algorand, ava, sui}, are actively developing and deploying BFT protocols~\cite{bullshark, spiegelman2023shoal, chen2019algorand, snowflake, jolteon}, to support the growing Web3 industry, with millions of users worldwide using these systems daily.

The pioneering BFT research~\cite{lamport2019byzantine, dolev1983authenticated, flp} primarily focused on theoretical feasibility across various communication and adversarial models. PBFT\cite{castro2002practical} stands out as the first academic BFT implementation, demonstrating the practical viability of BFT. This leader-based protocol requires three message delays to commit a leader's proposal in the common case, matching the lower bound for optimal resilience protocols.


Recently, due to the growing demand for high-performance decentralized blockchains, much of the research has been dedicated to improving BFT throughput and scalability. However, there has been a misconception that the primary objective is to reduce the message complexity of protocols~\cite{SBFT, tendermint, spiegelman2021search}, sometimes at the cost of increased latency~\cite{hotstuff}.


A breakthrough in BFT throughput occurred with the realization that load balancing and maximizing resource utilization are the key~\cite{narwhaltusk, MirBFT, arun2022dqbft}.
%more crucial than minimizing the total number of messages~\cite{narwhaltusk, MirBFT, arun2022dqbft}.
Narwhal\&Tusk~\cite{narwhaltusk} was among the first systems to embody this insight, showcasing over a 10x increase in throughput compared to state-of-the-art leader-based solutions~\cite{hotstuff, jolteon}. Unlike leader-based protocols, which are limited by leaders' bandwidth for broadcasting data, Narwhal is a leaderless system that achieves perfect load balancing of data dissemination among validators through a directed acyclic graph (DAG) construction.


In a nutshell, Narwhal constructs a round-based DAG where each node \sd{Node is a bit confusing and gives a feeling similar to validator. May be it is just me. An alternative is to use the term "vertex".} (1) contains a batch of transactions proposed by the associated validator and (2) links to $2f+1$ nodes in the previous round. 
Tusk is a consensus protocol that allows validators to locally interpret the DAG structure as a consensus logic and order all the nodes without requiring additional communication.
Some nodes are chosen to be anchors (aka leaders) and links in the DAG are interpreted as votes that commit the anchors. Non-anchor nodes are ordered as part of committed anchors' causal histories.  


While Narwhal\&Tusk's throughput was unmatched before, its major drawback is its high latency, which is unacceptable for modern Blockchains.
The high latency of Narwhal\&Tusk stems from two main factors. First, the nodes in the Narwhal DAG are \emph{certified}. That means that validators aggregate a quorum certificate on their nodes before disseminating them to be added to the DAG, which leads to an additional round trip for every node broadcast \sd{are you doing a reliable broadcast?}. Second, Tusk's algorithmic commit logic is sub-optimal and does not effectively compensate for the high broadcast latency.

%So we want to keep certification for overall performance.
To improve Narwhal's latency, one approach is to eliminate the node certification step and construct the DAG directly with raw nodes~\cite{keidar2022cordial, mysticeti}.
%, broadcasting roughly every message delay~\cite{keidar2022cordial, mysticeti}. 
However, this approach has practical drawbacks as it results in a fragile DAG construction. Byzantine validators can equivocate by sending different nodes to different validators and it cannot efficiently handle faulty and slow validators, resulting in higher latency.\sd{Do you want to say that prior works such as \cite{keidar2022cordial,mysticeti} has bad worst case latency, but better optimistic latency? It does not come out clearly here.} As explained in more detail later, while certifying nodes adds extra time, the resulting DAG allows fetching missing nodes off the critical path and with a better load balancing. %, ultimately reducing the overall latency. 

Another approach to reducing latency is by improving the DAG's local ordering logic, as was previously done in Bullshark\footnote{Bullshark and Narwhal are currently deployed on the Sui Blockchain~\cite{sui}. }~\cite{bullshark, bullsharksync} and Shoal~\cite{spiegelman2023shoal}.
Bullshark reduces Tusk's anchor commit latency by 50\% by relaxing the networking assumption to partial synchrony, which is the common assumption in practice.
Shoal further reduces latency by introducing pipelining to the Bullshark protocol, ensuring an anchor for each round instead of every second one.
This results in an average node latency of 9 message delays.

To get a sense of how much further the Shoal latency can be improved while preserving its high throughput, it is important to compare it to what can be achieved with leader-based protocols.
While vanilla leader-based protocols cannot match Shoal's throughput, they can be enhanced with a load-balanced data dissemination mechanism to optimize resource utilization, as demonstrated in the Aptos Blockchain with the Quorum Store mechanism~\cite{quorumstore}. 

In a nutshell, Quorum Store is incorporated sequentially before consensus, mirroring the node certification and broadcast process in the Narwhal DAG.
%Validators continually stream data batches, create batch certificates, and broadcast these certificates (small metadata) to all validators for proposal in consensus. 
This layer introduces an additional delay of 3 messages to the consensus latency, so an integration with a latency optimal protocol such as PBFT results in overall 6 message delays. \sd{I agree with Florian. I am not sure if the discussion about Quorum store necessary here.}
%integrated with Jolteon, the current consensus protocol deployed on Aptos, the total delay is 8 messages, while the theoretical limit could be reduced to 6 with an optimal latency protocol like PBFT.



Therefore, the Shoal protocol has a latency gap, as it is possible to have a system with better latency and comparable throughput. In fact, such a Byzantine fault-tolerant (BFT) system is currently deployed on the Aptos Blockchain.

The question we address in this paper is: How much further can we reduce the latency of Narwahl-based BFT consensus? Is it feasible to maintain the perfect load balancing and high throughput of the Narwhal DAG construction while achieving the best possible latency of vanilla leader-based consensus protocols like PBFT?

\sd{The writeup so far seems to be very targeted towards an expert who is familiar with the works you list through. It will be nice to give a slightly higher level picture to non-experts.}
\fs{I agree -- I will propose a re-write soon that is more accessible to a wider audience}

\subsection{Our contribution}
\fs{I've not read the "pratical section in detail", but it seems to me that some of those are actually actively informing the protocol and should go into the main section. (I'm specifically thinking S5.2, S5.3 and S5.4}
\fs{making notes (commented) our for some re-write}
\iffalse
Skip straight to section two (merge this and current S2). Call it "Dissecting DAG Latency". Three blocks
1) DAG introduction. This needs to come FIRST as context => DAGs displace leader based designs by focusing on max utilization. (Note: should acknowledge multi-leader frameworks; BFT MIR was also at Eurosys: https://dl.acm.org/doi/pdf/10.1145/3492321.3519579)
2) Latency analysis/breakdown into the three components. (and what is the optimal)
3) Our key ideas, one for each component. 
    a) improve commit speed of leader; by small trick on commit rule => this benefits all block latency
    b) improve commit latency of non-leaders =>  This one addresses BOTH sibling and queuing latency...
        i) improve sibling latency (non-leaders in leader round
        ii) increase frequency of leaders to be every message delay (pipeline) => avoids missing the bus + no "gap rounds"
        (Note: Shoal already improved to having leader per round, rather than every 2 rounds. But latency is still on avg 9md)
   
    

\fi

This paper considers the end-to-end latency, starting from when a transaction reaches a validator to when it is ordered. \fs{I'd replace all validator mentions with "replica". Be general BFT, avoid blockchain "slang"}
While many academic studies consider latency as the time taken for a system to commit a proposal, we extend our analysis to consider the queuing time, which also includes the waiting time for a transaction to be included in one. 
Note that the queuing time, which directly influences the latency experienced by clients, might be significant even under low load due to the time gap between two consecutive proposals.\fs{this observation of a bottleneck needs to be in the intro already.}

\fs{TODO: FIRST need a short background section where DAG is roughly explained. THEN break it apart into targets}

We divide the DAG BFT latency into three components: \fs{nit: paras should be in same order as enumeration}
\begin{enumerate}
    \item \textbf{Queuing latency:} the time for a transaction to be broadcasted as part of a node.
    \item \textbf{Sibling latency:} the time to incorporate a non-anchor node into an anchor's causal history.
    \item \textbf{Anchor latency:} the time to commit an anchor.
\end{enumerate}

% We present \sysname, a narwhal-based BFT system that reduces latency in each of these components. While supporting the throughput of Narwhal, \sysname achieves a theoretical end-to-end latency of 4.5 message delays in the common case, improving on Shoal by 6 message delays.
% For comparison, the best we can achieve with the fastest (but low throughput) leader based BFT is 4 message delays  (excluding queuing) -- 3 to commit a leader's proposal and 1 to propagate transactions to the leader.

\fs{wouldn't say again it's Narwhal based, but generalize to DAG BFT -- saying it once in intro is enough I think. Once may be good since it was best paper at Eurosys before though.}
We present \sysname, a narwhal-based BFT system, designed to minimize latency across all components. \sysname not only sustains the high throughput of Narwhal but also achieves an end-to-end latency of 4.5 message delays in the common case, surpassing Shoal's latency by 6 message delays. For comparison, even the fastest low throughput leader-based BFT protocols cannot commit in less than 4 message delays (excluding queuing) -- 3 delays to commit a leader's proposal and 1 delay to propagate transactions to the leader.


\paragraph{Anchor Latency.} \sysname's algorithmic contribution is reducing the anchor commit rule in Bullshark from 6 to 4 message delays. The direct commit rule in Bullsahrk requires $f+1$ certified nodes to link to the anchor.\fs{definitely needs } We observe that an anchor can be committed as soon as $2f+1$ uncertified nodes linking to it are received. The new commit rule is Safe since at least $f+1$ out of these $2f+1$ uncertified nodes were sent by honest validators and will eventually be certified.

\paragraph{Sibling latency.}
Most of the nodes in DAG BFT consensus are not anchors and ordered as part of anchors' causal histories. In Narwhal based protocols, for example, it take 3 message delays more to order a non anchor node.   
The Shoal paper explains how to extend their pipelining idea to multiple anchors per round, potentially cutting this extra latency. 
However, as we explain later, the proposed solution was not practical and therefore never implemented. \fs{do not have a forward reference; needs to be explained now. --> should be easy to address with my proposed re-write structure. Side note: I assume you are implicitly referring to what they do in Mysticeti with multiple leaders per round? Or what is the context?}
In brief, even one slow anchor can increase latency for all others in a round, resulting in a worst overall performance.

In \sysname, we solve this problem on the system level. First, we use leader reputation to filter out anchors associated with slow validators. \fs{This I would move only to a later optimization section.}
Second, we use (small) timeouts to slightly slow down the DAG construction to let slower validators the opportunity to catch up.

Reducing system latency by slowing down validators and giving up optimistic \changebars{responsiveness}{repulsiveness} \fs{repulsiveness is great though :)} (network speed) is perhaps surprising and counterintuitive.
%This is perhaps surprising and contra-intuitive that we reduce the system latency by slowing down validators and giving up optimistic repulsiveness (network speed). 
%The reason it works is that even though each round in the DAG takes slightly longer, \sysname is able to treat most nodes as anchors and thus commit them with fewer DAG rounds.
It works because, although each round in the DAG takes slightly longer, \sysname can treat most nodes as anchors, enabling it to commit them with fewer DAG rounds. \fs{it's not clear what the actual idea/mech is here}

%It is important to distinguish between the round timeouts used in \sysname and the view timeouts used in leader-based protocols. While the round timeout in \sysname is solely for performance and can be arbitrarily small, the view timeout is necessary for liveness and is very tricky to optimally set. \sysname adopts the approach proposed in Shoal and leverages the DAG construction to eliminate view timeouts.
%\sasha{the above should maybe move to related work.}

\paragraph{Queuing latency.}

Since it takes 3 message delays to certify a node and advance a round in Narwhal, a transaction waits, on average, 1.5 message delays to be proposed even under low load. In \sysname, we propose a novel approach to reduce the average queuing delay to 0.5 message delays. \fs{do you mean RT and not md? i.e. 1.5RT = 3md?}\fs{I think talking about average in a non-formal context is a bit confusing, but it's just my personal opinion. I would say "up to 3 message delays" and "at most 1 md". I also don't understand where the averages even come from? n-1 nodes experience 3md, and 1 (the leadeR) experiences 0. And with pipleine it is n-1 see 1md, and 1 sees 0md? }
The idea is to build three DAGs, run three instances of the protocol in parallel, and alternate between their committed nodes. This way, if the instances offset by roughly one message delay, validators propose new nodes
%and nodes are being ordered 
every message delay. 

Theoretically, we could maintain any number of instances, thereby arbitrarily reducing the queuing latency. However, in practice, as we explain later, it is not clear how to synchronize more than three DAGs.
\sasha{revisit this after we make 3 DAGs work.}


In summary, to put our contributions in a broader context, the anchor optimization is specific to Narwhal-based BFT, the sibling optimization is for any round-based DAG BFT, and the queuing optimization can be applied to any BFT protocol, including leader-based ones.

We integrated our production-grade implementation of \sysname in one of the major Blockchain open source projects and evaluated the system in production-like decentralized environment. We compared \sysname to Shoal, Bullshark, and Jolteon~\cite{jolteon} enhanced with Quorum Store~\footnote{Currently deployed on the Aptos Blockchain}. %\fs{don't need to mention which exact systems here} 
Our results show that ...  







==> sections/2-background.tex <==
\section{DAG BFT} 
\label{sec:dagbft}

In this section, we describe the system model and provide the necessary background to understand the \sysname protocol.
%and contribution. 

\subsection{Model, problem statement, and assumptions}
\fs{would move model to it's own section later, right before the full formal protocol}

The goal of a BFT system is to allow a set of validators to continuously propose transactions and to agree on an ever-growing ordered log of them. We consider a traditional setting of a peer-to-peer message-passing network comprising $n$ validators, with a computationally bounded adversary. We design \sysname to be secure under worst-case assumptions while optimizing it for the common case. \sysname guarantees that validators never disagree on prefixes of the log (Safety) against an adversary that has full control over the network and can corrupt up to $f < n/3$ \emph{Byzantine} validators. Theoretical liveness, ensuring that the log eventually grows, is guaranteed in partially synchronous networks in which there is a global stabilization time after which messages arrive within a bounded delay. The practical latency of \sysname for transactions to be included in the ordered log, however, is optimized for the crash-failure case, in which validators are not corrupted but may crash or be extremely slow. 


\subsection{Background}

In Section~\ref{sec:related} we provide a detailed overview and comparison of the DAG BFT literature, but here we focus on the prior work that shaped the \sysname design.   

\fs{I'd change para naming to be "DAG structure/core", and "Consensus on DAG" (instead of breaking it into Narwahl/Bullshark/Shoal pieces)}
\paragraph{The Narwhal DAG}

Narwhal~\cite{narwhaltusk} is one of the first BFT systems to overcome the throughput bottleneck of traditional leader-based consensus, in which the overall system throughput is bounded by the ability of a single leader to disseminate data.
Narwhal, in contrast, is a leaderless load-balanced system in which all validators perform the same amount of work, perfectly utilizing the system resources.

At the core of the Narwhal design is a round-based DAG. 
Each round in the DAG contains at most $n$ certified nodes, one per validator. 
Each certified node in the DAG contains transactions and links to $n-f$ nodes from the previous round.
To add a certified node to the DAG in round $r$, a validator needs to receive $n-f$ certified nodes in round $r-1$ (in its local copy of the DAG) and follow the following:
\begin{enumerate}
    \item create a node in round $r$ that links to $n-f$ certified nodes from round $r-1$ and broadcasts it
    \item once a node in round $r$ is received, sign it and send the signature back to the sender if no contradicting node from the same author was already signed in round~$r$
    \item wait to receive $n-f$ signatures back and form a certificate 
    \item broadcast the certified node 
    \item once certified node is received add it to the local copy of the DAG
\end{enumerate}
\fs{Add a sentence: This protocol guarantees that all replicas eventually see the same DAG. (i.e. it is equivocation free and each node is available for sync). Then for consensus its easy to say: "since DAGs are the same, its enough to interpret the local view -> no extra messages need to be exchanged"}

Figure~\ref{fig:narwhaldag} illustrates a DAG of certified nodes as it appears in a local view of one of the validators. 
Figure~\ref{fig:narwhalround} illustrates the creation of certified nodes.\fs{I don't understand figure2, it's visually quite confusing. Maybe you could draw a single unified figure in which there is a "zoom in" on what happens inside one DAG "round"}
 
\begin{figure}[h]
    \centering
    \includegraphics[width=0.4\textwidth]{figures/narwhaldag.pdf}
    \caption{Narwhal's round-based DAG from a validator's local point of view. All nodes are certified.}
    
    \label{fig:narwhaldag}
\end{figure}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.4\textwidth]{figures/narwhalround.pdf}
    \caption{One round on the DAG from a validator's local point of view. The validator receives uncertified nodes pointing to $n-f$ certified nodes in the previous round, signs them, sends back the signatures, and later gets the nodes' certificates.}
    
    \label{fig:narwhalround}
\end{figure}

The advantage of certified nodes is twofold: first, it eliminates the ability of Byzantine validators to equivocate and thus simplifies the DAG ordering logic, and second, it provides Poof of Availability~\cite{cohen2023proof, quorumstore} for the ancestors' nodes, which makes DAG fetching and data streaming much simpler (see more discussion in Section~\ref{sec:practical}). 
\fs{it also makes it more robust in a principled way (see Autobahn)}

\paragraph{The Bullshark consensus protocol.}
Bullshark~\cite{bullshark, bullsharksync}, is a consensus protocol, currently running in production on the Sui~\cite{sui} Blockchain, designed to order the nodes in a narwhal-based DAG without communication among the validators. 
That is, validators collectively build a DAG as described above and then interpret their local copies of the DAG as a consensus logic. Some nodes are interpreted as proposals, and links are interpreted as votes. 

In Bullshark, there is a pre-defined anchor (aka leader) node in every other round. 
An anchor is directly committed with $f+1$ votes, or in other words, when there are $f+1$ nodes in the next round that link to it.
A validator traverses the anchors in its local DAG, starting immediately after the last committed anchor $A$, until some anchor $A'$ is directly committed. 
Since validators may have slightly different local views of the DAG, some validators may directly commit anchor $A$ (or some other anchor in between) before $A'$.
Therefore, the protocol ensures all validators commit that anchor before $A'$.
After validators agree on what anchors to commit, they traverse them one by one and deterministically order their causal histories.  

The details of the Bullshark logic to agree on what anchors to commit is not necessary for understanding the contribution of this paper and a curious reader is referred to~\cite{bullsharksync}. 
However, it is important to emphasize that:
\begin{itemize}
    \item There is a pre-defined anchor in every other round
    \item An anchor is directly committed with $f+1$ votes
    \item An anchor needs two DAG rounds to be (directly) committed in the common case.
    \item In the bad case, when an anchor cannot be directly committed, validators need more DAG rounds to determine whether the anchor should be committed.
    \item non-anchor nodes are ordered as part of committed anchors' causal histories.
\end{itemize}
%
Figure~\ref{fig:bullshark} illustrate the anchors' commit logic in Bullshark.
%
\begin{figure}[h]
    \centering
    \includegraphics[width=0.4\textwidth]{figures/Bullshark.pdf}
    \caption{Bullshark anchors' commit logic. Validator 4 has two $2=f+1$ votes for anchor A1 in his local view of the DAG, and thus directly commits it. Validator 1 has only $1 < f+1$ vote, and thus cannot directly commit A1. Therefore, when validator 1 directly commits A2, there is a logic on the DAG to ensure that $A1$ is committed before $A2$.}
    \label{fig:bullshark}
\end{figure}



\paragraph{Shoal latency improvements.}
Shoal~\cite{spiegelman2023shoal} builds on top of Bullshark to reduce its latency. The two main algorithmic contributions of Shoal are leader reputation and pipelining. 

The leader reputation mechanism elects future anchors based on validators' past performance. This significantly reduces latency in practice since crashed or slow validators do not slow down the overall system's progress.

The pipelining mechanism allows Bullshark to run with an anchor in every round, reducing the common case latency. The Shoal paper also mentions that, in theory, the same technique can be applied to have multiple anchors per round, but the paper does not provide an implementation or description of how it can be done in practice. 
%More details about the practical challenge and how \sysname overcomes it are given in Section~\ref{sec:practical}.

On the system level, Shoal is the first deterministic BFT protocol to eliminate leader timeouts~\footnote{In all but a few extremely unlikely scenarios.}. The protocol takes advantage of the asynchronous DAG construction and the leader reputation mechanism to guarantee network speed progress under most failure and networking scenarios. A property they call \emph{Prevalent responsiveness}. We adopt this technique in \sysname. 


\subsection{Latency}

The best theoretical latency one can hope for in a BFT system is three message delays~\cite{castro2002practical}. However, the only protocols that achieve it as of today are leader-based, where the overall system throughput is bounded by the leader's ability to disseminate data. 
To unlock high throughput in BFT system, data dissemination has to be parallelized. \fs{I would not mention the Quorum store approach. It lacks context and will just confuse. It can be left to the evaluation section as an example of robustly separating data dissemination with traditional BFT} There are currently two deployed approaches. One is to have a data availability layer~\cite{quorumstore} before consensus, as the one currently used at Aptos~\cite{aptos}, which adds another 3 message delays to the system.
The other approach is to use DAG BFT as the symmetric and leaderless DAG construction mechanism fits perfectly for parallel data dissemination. 

The goal of this paper is to push the limit of DAG BFT latency to match the best possible with leader-based protocols while maintaining a high throughput.

\fs{can cut everything that's redundant}
The overall theoretical latency of DAG BFT systems, from the time transactions are submitted until the time they are ordered, can be broken down as follows:
%
\begin{enumerate}
    \item \textbf{Queuing:} The time transactions wait to be included in a node.
    \item \textbf{Sibling latency:} The time for a non-anchor node to be included in an anchor's casual history.
    \item \textbf{Anchor latency:} The time for an anchor node to be committed.
\end{enumerate}
%

\fs{might be nice to have a table that compares the breakdown in different protocols? (this will show that Shoal improves only 1 axis, but this work does 3}
Figure~\ref{fig:latency} illustrates the latency breakdown in the Shoal consensus protocol in the good case.
\textbf{Queuing:} Since it takes three message delays to add a node to the Narwhal DAG (broadcasting the node, aggregating signatures, and broadcasting the certified node), a new transaction entering the system waits, in expectation, 1.5 message delays to be included (broadcasted) in a node. \fs{again, saying/showing 1.5 md is very weird in a figure that implicitly is a happens-before-relation}
\textbf{Sibling:} Most nodes in the DAG are non-anchor nodes and are committed as part of an anchor's causal history. Since Shoal has an anchor in every round, it takes a non-anchor node one DAG round (three message delays) to be linked by an anchor.
\textbf{Anchor:} In the good case, an anchor node is committed in two DAG rounds (six message delays). One round is needed to add the anchor to the DAG, and another round is required to add the vote nodes.
%
\begin{figure}[h]
    \centering
    \includegraphics[width=0.48\textwidth]{figures/shoallatency.pdf}
    \caption{Breakdown of Shoal latency. Transaction $tx$ arrives at validator 2 at time $t_1$. Validator 2 includes $tx$ in a node and broadcasts it at time $t_2$. The node is added to the DAG and linked by the next anchor at time $t_3$. The anchor is committed at time $t_4$.}
    \label{fig:latency}
\end{figure}

The overall Shoal theoretical latency is 10.5 message delays.  \fs{Isn't Bullshark 10.5, and Shoal 9?. Worst-case bullshark has 12 (sibling nodes), and 9 (non-anchor rounds). Shoal every round in anchor, so there is only sibling latency = 9}
As described in detail in the next sections, \sysname cuts the queuing latency to 0.5 message delay, eliminates the sibling latency, and cuts the anchor latency to 4 message delay. Overall the \sysname total theoretical latency is 4.5 message delays, which is more than x2 (6 message delays) better than Shoal.

==> sections/3-Shoal++.tex <==
\section{\sysname: Algorithmic Overview} 
\label{sec:overview}
\fs{Re-structure: After S2 that sets the tone have a quick overview section. Then the model. Then a *detailed* protocol section without forward references to some later practical consideration. Only then proofs (if any)}

In this section, we explain the algorithmic contribution of \sysname.
We consider the end-to-end consensus latency from when a validator receives a transaction until the transaction is ordered, which in the DAG BFT case includes 3 phases: queuing, sibling, and anchor latencies. 
Below we describe how \sysname improves latency in each of these phases.
We name \protocolname the protocol enhanced with the anchor and sibling optimizations.  

%The pseudocode of \sysname's protocol appears in Algorithms~\ref{}.

\fs{Soft opinion: I usually like when the protocol section is readable in a "self-standing" manner. That means it should brielfy "re-explain" how the DAG is built, how leaders are chosen etc., how consensus works, how the Dag is redued to a total order, etc. Describing it bottom up, and highlighting what parts are "new/better" is better for a general audience -- currently it says "these are the modifications we make" which only works for people already very familiar} \fs{concretely: In the background section I'd leave the DAG description more "rough", and instead put the precise description here (while saying this part is just taken from Narwhahl/Bullshark)}

\subsection{Anchor latency: faster direct commit rule}

As described in the previous section it takes 6 message delays to commit an anchor in Bullsahrk and Shoal in the common case. One DAG round for the anchor node and one DAG round for the vote nodes, where each round in a Narwhal-based DAG takes 3 message delays.
The commit rule in Bullshark and Shoal is $f+1$ votes. i.e., $f+1$ nodes in the voting round that point to the anchor.

We observe in \sysname that we do not need to wait for the $f+1$ certified vote nodes to be added to the DAG. Sometimes we know in advance that it will eventually happen.

Recall (Figure~\ref{fig:narwhalround}) that in a narwhal-based DAG, each validator, in each round, first broadcasts a node, and then collects a quorum certificate and broadcasts the certified node again to be added to the DAG. 
Therefore, if a validator receives $2f+1$ (uncertified) nodes that link the anchor, then at least $f+1$ of these nodes were sent by honest validators and will be eventually certified and added to the DAG.

Hence, a validator can safely commit an anchor after seeing $2f+1$ nodes that link to it, reducing the anchor latency to 4 message delays in the good case: 3 to add the anchor to the DAG and 1 more to broadcast the vote nodes.
A formal security proof for this optimization is given in the next section.

It is important to note that it is possible in certain cases to get $f+1$ links from certified nodes faster than getting $2f+1$ links from uncertified nodes. 
Therefore, we combine both commit rules in \sysname so validators can directly commit anchors with whatever rule is satisfied first.
However, as supported by our evaluation in Section~\ref{}, Bullshark's commit is rarely triggered and validators take advantage of the new commit rule most of the time. 
Figure~\ref{fig:commitrule} illustrates both direct commit rules. \fs{nice fig.}
%\sasha{maybe make the description in the previous section an Alg and refer to it here.}


\begin{figure}[h]
    \centering
    \includegraphics[width=0.4\textwidth]{figures/commitrule.pdf}
    \caption{Bullsharks's direct commit rule requires f+1 certified vote nodes, while \sysname's direct commit rule requires $2f+1$ (uncertified) vote nodes.}
    \label{fig:commitrule}
\end{figure}



\subsection{Sibling latency: multiple anchors per round}

As described above, it takes 3 extra message delays for non-anchor nodes to be ordered since they are ordered as part of anchors' causal histories.
In \sysname we eliminate this latency by having multiple anchors per round.

\fs{this whole para is quite confusing, and the forward reference is not helpful. Should describe directly how it's made to work. Just so I understand though: This is the exact same as in Mysticeti?}
The Shoal paper explains (without implementation) how to, in theory, extend their pipelining idea to multiple anchors per round.\fs{I would not say this.}
The idea is simple, every node in the DAG is treated as an anchor, and for every anchor, validators interpret the DAG as a single shot Bullshark instance.
If the Bullshark instance determines that the node (anchor) should be ordered (either with a direct or indirect commit), then the node and all its (yet-to-be-ordered) causal history are ordered immediately.
Otherwise, the node might be ordered as part of some future anchor's causal history.  
This way, in the best case (at least in theory), every node in the DAG is ordered with an anchor latency.


In practice, however, this idea will not work if done naively. 
Recall that for a slow validator, it might take many rounds to decide whether to skip or order the anchor associated with it (see Figure~\ref{fig:bullshark} for an example).
If we consider all nodes to be anchors, with a high probability we will have at least one such slow anchor in every round. 
Now since the order in which the anchors' Bullshark instances are run in each round has to be deterministic across all validators, a slow anchor will stall the progress of the whole protocol.
This is because an anchor that necessitates more rounds incurs a latency penalty for the subsequent anchors in the round.


The Shoal paper also suggests using its leader reputation mechanism to elect the nodes that should be considered anchors in each round.
The hope is that nodes associated with slow or faulty validators will be filtered out, allowing the protocol to directly commit all anchors with best-case latency.

We adopt this idea in\sysname and extend Shoal's leader reputation mechanism to support multiple anchors per round, but unfortunately, we observed that it cannot, by itself, overcome the unpredictability of a geo-replicated distributed system.
In Section~\ref{sec:practical} we describe how we made this optimization work in practice in \sysname.   
\sasha{TODO: explain there the round timeout and contrast with a leader timeout that we do not have}

Figure~\ref{fig:multipleanchors} illustrates Shoal's idea of multiple anchors per round and the problem in its naive implementation.

\begin{figure}[h]
    \centering
    \includegraphics[width=0.4\textwidth]{figures/multipleanchors.pdf}
    \caption{All nodes are considered anchors and the DAG structure is reused to order (or not) each one of them with a dedicated Bullshark instance. To satisfy determinism, decisions are made in a pre-defined order. In the best case, all anchors (nodes) are directly committed. In the bad case, one slow validator imposes latency on all anchors. In this example, the blue anchor is considered first and ordered fast since it can be directly committed with $3 \geq f+1$ votes in its instance. However, the green and the pink anchors must wait two extra rounds for the orange to be (indirectly) committed even though they are committed directly in their Bullshark instances.}
    \label{fig:multipleanchors}
\end{figure}


\subsection{Queuing latency: 3-DAGs in parallel}

\balaji{I think we should explain why only 3 DAGs. PBFT proposed to do many rounds in parallel.}
\fs{+1. Note to self:"consensus should only run when there is new available data" -> Pipeline dags to have 1 each round. Given dag latency, this adds up to max 3 active dags in practice. More is useless}

As explained above it takes 3 message delays for a validator to propose a new block in a Narwhal-based BFT protocol. Thus the average queuing latency for a transaction is 1.5 message delays. 
In \sysname, we reduce this latency to 0.5.

The idea is simple. \sysname maintains 3 DAGs and runs 3 instances of the \protocolname protocol in parallel.
Think of each instance of \protocolname as a black box that continuously outputs sets of ordered nodes.
The total ordering is done in a round-robin. Validators start by ordering the first output of the first instance. Then they order the first output of the second instance followed by the first output of the third instance. 
Then, they order the next output of the first instance, and so on.

Safety and liveness follow from the corresponding safety and liveness of each \protocolname instance together with the deterministic manner of the round-robin process.   

In theory, we can reduce the queuing latency as close to zero as we want by adding more and more DAGs, but the practical challenge is how to synchronize and offset them to achieve the desired queuing latency.
\fs{I assume in the later section you talk about the subtelty with using "votes" as a new proposal?}

\sysname uses 3 DAGs so a node is broadcasted (and committed) every message delay, reducing the average queuing latency to 0.5.
Figure~\ref{fig:threedags} illustrates the 3 DAGs synchronization in \sysname and in Section~\ref{sec:practical} we describe it in detail.


\begin{figure}[h]
    \centering
    \includegraphics[width=0.4\textwidth]{figures/threedags.pdf}
    \caption{Three dags. Dashed squares are nodes. 
    Solid squares are certified nodes. \sysname synchronize the DAGs in a one message delay offset.} 
    \label{fig:threedags}
\end{figure}


\subsection{Pseudocode}

In this section, we describe the pseudocode of \protocolname and \sysname as presented in Algorithms~\ref{alg:dagapi} to \ref{alg:shoalpp}.

\input{code/dagapi}

Algorithm~\ref{alg:dagapi} presents the node structure and the DAG API that we assume. For the sake of brevity, we do not duplicate the pseudocode that is available in previous works and, in particular, omit the description of the DAG construction (i.e., node broadcasts, transaction submission, node fetching, garbage collection, and so on).%\fs{I think you should have it, and only omit things like synchronization/garbage collection}

The procedures \textsc{process\_node}, \textsc{process\_certified\_node}, and \textsc{causal\_history} are logically similar to Narwhal.
As for timeouts, similarly to Shoal we eliminate leaders' timeouts in the DAG construction but add a shorter timeout 
to each round to ensure validators move roughly at the same pace (see more details in Section~\ref{sec:practical}). 

The procedure \textsc{run\_bullshark} runs the Bullshark logic to interpret the DAG as a binary consensus on a given anchor. It returns true if the anchor is ordered by Bullsahrk and false if it is skipped.

The procedure \textsc{get\_anchors} implements the leader reputation logic we use in \sysname. For a given round, it returns a vector of nodes to be considered as anchors. Similarly to the mechanism in Shoal, it is based on validators' performance. 

\input{code/mako}

Algorithm~\ref{alg:mako} presents \protocolname, which includes the anchor and sibling latency optimizations of \sysname.
Validators maintain a data structure weak\_votes to count the number of links from uncertified nodes each node in the DAG has, which is updated every time an uncertified node is received.

The procedure \textsc{fast\_commit}($n$) returns when the node $n$ accumulates $2f+1$ links from uncertified nodes.

The procedure \textsc{next\_ordered\_nodes} is called from the outside and returns a vector containing the next ordered anchor and its causal history.

The procedure traverses all anchors in a round in a deterministic order, starting from the last ordered one, until an anchor is ordered. To check if an anchor should be ordered, the procedure calls in parallel to  \textsc{fast\_commit} and dag. \textsc{run\_bullshark} and adopt the first response. In the next section, we prove that the calls never return contradictory values.
In Section~\ref{sec:practical}, we explain a more practical way to implement the Sibling (multiple anchors per round) latency optimization.
 

\input{code/shoalpp}

Algorithm~\ref{alg:shoalpp} presents the queuing latency optimization of \sysname on a high level. It maintains three different instances of the \protocolname protocol (respectively, three different DAGs) and deterministically outputs their next ordered nodes in a round-robin manner. In Section~\ref{sec:practical} we provide more practical details,
 



==> sections/5-practical.tex <==
\section{\sysname: Practical Consideration} 
\label{sec:practical}
\fs{I think the only things in this section should be: Efficient fetching, Inline data streaming, distance based priority, and leader reputation. Effective message delay + 5.2/5.3/5.4 should go into the main section. => Rename this section to Practical Optimizations, OR put it into the implementation section}

\sasha{Balaji's idea of sending optimistic votes.}

In this Section, we provide some of our design choices while implementing \sysname. We split the presentation according to the protocol's components.  

\subsection{DAG construction}

\paragraph{Certified nodes.}
As first proposed by Cordial Miners~\cite{keidar2022cordial} and later implemented by Mysticiti~\cite{}, it is possible to run PBFT~\cite{} on an uncertified DAG.
This, at least from a theory point of view, can reduce the anchor latency to 3 message delay, matching the lower bound. 

However, in \sysname, we choose to keep the original design of Narwhal that requires 3 message delays to add a node to the DAG, leading to an anchor latency of 4 message delays.
Although it looks like we are sacrificing 1 message delay in the latency, we get more back by having a more reliable DAG construction:
 \fs{I'd call these "robust/predictable Latency" and load balanced synchronization}
\begin{itemize}
    \item \textbf{Effective message delay is faster.}A node certificate provides a proof of availability of the nodes' parents and the data therein. Therefore, a validator can advance to round $r+1$ and broadcast a new node as soon as $2f+1$ certified nodes are delivered in round $r$.
    Hence, if some nodes or data are missing, they can be fetched outside the critical path. 
    Moreover, to certify a node, a validator does not depend on other validators broadcasting theirs.\\
    
    In an uncertified DAG, however, the proof of availability is coupled with the DAG structure. This means that a validator links to a node only if it has all the nodes' causal history. 
    Otherwise, it will need to fetch first, stalling the DAG construction by at least two extra message delays per round.
    So even for an honest validator, if its node links to nodes that other validators do not locally have (the validator cannot possibly know), then validators will not link to it until they fetch the missing nodes.  
    As a result, the best latency the protocol can achieve with even one Byzantine validator in the system is $3x3=9$ message delays for an anchor.\fs{3md per round, at 3 rounds} In practice, in a wide area network, validators are likely to struggle to advance rounds even without Byzantine behavior, increasing the "effective" message delay. 
 
    \item \textbf{Efficient fetching}
    The node certificate not only provides proof of availability but also a bitmap of validators that signed it. This allows to load balance of the fetching mechanism as validators can choose any subset of validators from the bitmap.\\
    \fs{clearer: a certificate proves that f+1 correct replicas have the data; it can thus be fetched (in a load balanced manner) from any f+1 subset (optimistically maybe we ask fewer), rather than from the sender. }

    In an uncertified DAG, in contrast, all validators fetch a node's causal history from the node's validator. This makes the problem above even worse, as the validator becomes a bottleneck.

\end{itemize}
An illustration of the uncertified DAG's latency issues appears in Figure~\ref{fig:uncertifieddag}.


\begin{figure}[h]
    \centering
    \includegraphics[width=0.4\textwidth]{figures/uncertifieddag.pdf}
    \caption{Solid squares represent nodes that are locally available to validator 1, out of which the black squares represent its local DAG. In an uncertified DAG, validator 1 cannot advance to round 2 and broadcast node $n''$ until node $n'$ is added to the DAG. But $n'$ cannot be added to the DAG until node $n$ is received. This is because no certificate proves its existence. In this example, validator 3 behaves honestly, and yet its node cannot be added, and the DAG construction stalls. 
    Moreover, to fetch node $n$, all validators have to contact validators 3 or 4 (who become a bottleneck) as there is no information about who else has the node.} 
    \label{fig:uncertifieddag}
\end{figure}

\paragraph{Inline data streaming}
\fs{notes: workers allow you to scale tput horizontally by adding more machines. For robustness however, this requires them to RB first. Since the tput we get is already so high (beyond what any Blockchain uses) we opt to run without workers. This saves some latency. Further, instead of streaming data, we opt to include it inline in the data proposal to avoid separate fetching. The parallel DAG structure makes it so we are sending out batches more often, so there is little loss here. }
The main observation in Narwhal is that data dissemination should (1) be de-coupled from consensus logic and (2) fully utilize networking resources.
Therefore, to push the limit of throughput and to support a scaling-out architecture, the Narwhal design consists of workers that continuously stream batches of data and primaries that construct a DAG containing the batches' digest.
The latency issue with this approach resembles the one described above. Validators cannot sign an uncertified node until they have all the batches corresponding to the node's digest, which sometimes leads to fetching data on the critical path.

In \sysname, we slightly sacrifice Narwhal's throughput to improve latency.
\sysname do not have workers and do not separate batches from digests. Instead, nodes directly include the data, and therefore, no data fetch is ever required.
The DAG structure guarantees that data is still disseminated in parallel, and with the queuing optimization, new data is broadcasted every message delay, which together archives almost full networking utilization.

\paragraph{Distance-based priority broadcast.}
We've noticed that in a system with 100 validators, broadcasting a message can consume a considerable amount of CPU time. Following a fixed arbitrary order can lead to certain validators consistently receiving the message last, increasing the risk of them falling behind.

To address this issue, in \sysname, each validator periodically measures the ping time to other validators. Based on these measurements, validators prioritize broadcasting to those that are farther away, helping to balance the message distribution and reduce the likelihood of certain validators consistently lagging behind.

\paragraph{Leader reputation}
\sasha{Do we want to say anything here?}
\fs{yes, I think this is a good place to talk about inheriting reputation from Shoal}

\fs{all of the below should go into the main protocol section}
\subsection{Anchor latency}

As mentioned in Section~\ref{sec:overview}, \sysname's direct commit rule combines two rules. Fast commit with $2f+1$ uncertified nodes or Bullshark commit with $f+1$ certified nodes. Although the fast commit can commit in 2 message delays faster than the Bullshark commit, we keep both.
This is because in practice, during unstable networking periods, the faster 34 validators percentage can move much faster than the 67 percentage, satisfying the Bullshark commit first.       

\subsection{Sibling latency}

In Section~\ref{sec:overview} we explain why the multiple anchors per round approach does not work if done naively. Below we present our practical solution.   
 

\paragraph{Round timeouts.}
\fs{describe "slot based"? all anchors are assigned an "order" in advance, can only order/execute once all preceeding have been committed. Question: what if they never are? => this is where skipping anchors comes in. (Round timeouts are to }
As explained above, even one anchor that cannot be directly committed stalls the progress of the rest of the anchors in the round.

The DAG construction, as explained in Narwhal and Shoal, advances in network speed. Once $2f+1$ certified nodes are received, validators can broadcast the next round's nodes.
Therefore, the DAG advances with the fastest 67 present of the validators, leaving the rest behind.
Note that a node can be only slightly slower than the fastest $2f+1$ nodes, and yet will not get enough votes to be directly committed.

Clearly, nodes associated with the lagging validators cannot be anchors.\fs{cannot -> shouldn't / it is preferable if not.}
This means that the best we can hope for is 67 percent of the validators contributing anchors in a round, leaving the rest of the nodes to be ordered as part of future anchors' causal histories.

Furthermore, due to the network instability in geo-distributed settings, the leader reputation mechanism cannot filter out the nodes (preventing them from becoming anchors) associated with the slow 33 percent of the validators.
This is because the set of the lagging validators keeps changing dynamically, which makes it hard for the leader reputation mechanism to perfectly predict an entire set of "strong" anchors. 
\fs{very confusing para. I assume you mean: Leader reputation can help a little, but not in a prinicpled way; the set of slow guys changes quickly, and even one slow guy can stall progress}


\sasha{Balaji, please verify the text below.}
To avoid this undesirable behavior, we introduce a round timeout in \sysname's DAG construction. In addition to waiting for the fastest $2f+1$ nodes, validators wait for a small timeout before advancing their rounds to let slower validators have the opportunity to catch up.

This might seem counterintuitive as it makes the DAG advance slightly slower. 
However, validators are more synchronized, and more nodes can satisfy the direct commit rule, and thus be anchors. 
So overall, even though the timeouts increase the effective message delay of the system, it allows \sysname to enable the multiple anchors per round optimization, which drastically reduces the average node latency as nodes need fewer rounds to be committed.
\fs{note: Timeouts help with slow replicas, but not with byz/crashed ones.}

Note that the round timeout in \sysname is different from the standard leader/view timeout.
While the leader/view timeout is often required to guarantee liveness in partial synchrony (w
e.g., synchronize between the views), the purpose of \sysname's round timeout is solely to improve performance.
As a result, it can be much more aggressive and thus we set it to be only slightly longer than 3  geo-replicated network message delays (the number of message delays required to add a node to the DAG). 

The Shoal paper was the first DAG BFT to show that due to the asynchronous nature of the DAG construction and since the "view-change" and "view-synchronization" mechanisms are embedded therein, the leader/view timeout can be eliminated in all practical network scenarios. 
We adopt the same approach in Shoal.

\paragraph{Skipping anchors.}
We explained above how we reduce the number of anchors that cannot be directly committed in \sysname.
However, it is impossible to completely avoid bad scenarios in practice, and sometimes \textsc{run\_bullshark} requires more DAG rounds to determine whether an anchor should be committed.
If an anchor $n$ in round $r$ is skipped, then there is some other anchor $n'$ in a round $r' > r$ that the Bullshark logic committed.
In this case, \sysname skips the rest of the anchors in round $r$ and jumps forward to round $r'$. This is because the DAG has enough rounds to directly commit the rest of the anchors in round $r'$ and most of the anchors in round $r$ are ordered as part of round $r'$ anchors' causal histories.   
\fs{I'm not following this description. + it should explain how this deals with crashed replicas (and byz?). Is this safe? Provide an argument}

\subsection{Queuing latency}

\paragraph{DAGs synchronization.}
\sysname builds three DAGs, in parallel. To achieve the best queuing latency, these DAGs need to be offset by exactly one message delay as illustrated in Figure~\ref{fig:threedags}.
To this end, we synchronize the DAGs' messages. 

There are three main types of messages in the DAG construction: node-broadcast, signature-reply, and certified-node-broadcast. 
In \sysname, a node-broadcast message of DAG $i \in \{0,1,2\}$ is sent together with the certified-node-broadcast message of DAG $(i+1)\%3$. The signature-reply messages are sent as fast as possible. 
This way, we ensure validators can get their nodes certified at network speed, but at the same time, the 3 DAGs advance roughly at the same speed, and new nodes are broadcasting every message delay.

To avoid transaction duplication across the DAGs, all three DAGs in \sysname share the same mempool. To increase concurrency, the DAGs use separate storage columns.   

\paragraph{Round latency}

It takes three messages to add a node to the DAG, but it is important to note the message delays are not the same as illustrated in Figure~\ref{fig:roundlatency}.

\begin{figure}[h]
    \centering
    \includegraphics[width=0.4\textwidth]{figures/roundlatency.pdf}
    \caption{Round latency. } 
    \label{fig:roundlatency}
\end{figure}

Validators must wait for $2f+1$ signatures before broadcasting a certified node and for $2f+1$ certified nodes before broadcasting the next round node. 
Singing the nodes, however, is done at network speed. 
Therefore, since \sysname synchronizes the DAGs by aligning the nodes and certified nodes broadcast, which both require roughly the same additional waiting time, the speed of each DAG construction is not significantly affected.

==> sections/6-implementation.tex <==
\section{Implementation} 
\label{sec:implementation}

\balaji{We only order nodes that have transactions to reduce VM overhead.}
TBD



==> sections/further.tex <==
\section{Further theoretical improvement}
With pipelining, \sysname introduces an anchor in every round. 
As a result, in the best case, each anchor requires 2 rounds to commit and while non-anchor vertices require 3 rounds.

In this section, we present an approach to further optimize the latency for non-anchor vertices.
In designing \sysname, we have crucially relied on the technique of retrospectively re-interpreting the DAG structure.
Taking this further, we could iterate over the vertices in each round in a deterministic order and treat each vertex as an anchor.
More specifically, for each vertex $v$, we can run an instance of the underlying protocol $\mathcal{P}$ (i.e., DAG-Rider, Tusk, and Bullshark) as a single-shot agreement with $v$ being the first anchor.
If $v$ is ordered by $\mathcal{P}$, we order it.
Otherwise, we skip.
In both cases, we ignore all other ordered/skipped anchors in this instance and move to the next vertex.
For every vertex $v$ we decide to order, we also order the previously skipped vertices in $v$'s causal history.
A pseudocode appears in Algorithm~\ref{alg:bounus}.

\begin{algorithm}
\caption{Single-shot Narwhal-based agreement for each vertex}
\begin{algorithmic}[1]
        \State $r \gets 0$
        \While{\emph{true}}
            \For{\textbf{each} validator $k$}
                \State let $v_{r,k}$ be a vertex by validator $k$ in round $r$
                \State let $F_{r,k}: R \rightarrow A$ be a known to all mapping from 
                \Statex \hspace{9.5mm} rounds to anchors such that $F_{r,k}(r) = k$
                \State execute $\mathcal{P}$, select anchors by $F_{r,k}$, starting from 
                \StateX\hspace{4.5mm} $r$ until the first ordered (not skipped) anchor $A$ 
                \StateX\hspace{4.5mm} is determined.
                \If $A = v_{r,k}$
                    \State order $A$'s causal history according to $\mathcal{P}$ 
                \EndIf
            \EndFor
        \State $r \gets r+1$ 

        \EndWhile
    
\end{algorithmic}
\label{alg:bounus} 
\end{algorithm}

In the theoretical best case, each vertex can be ordered in 2 rounds. 
However, in practice, some validators may be slower and, therefore, require more rounds.
This is because their corresponding single-shot instances would not be able to order them based on the "votes" in the subsequent round, and thus more rounds will be required to determine whether they should be skipped or ordered.
The issue arises because validators must process the vertices in a predetermined deterministic order. Consequently, each vertex that necessitates more rounds incurs a latency penalty for the subsequent vertices.

\sasha{figure?}

\paragraph{Combining with leader reputation}
The above issue can potentially be mitigated by combining it with the leader reputation mechanism.
That is, instead of running a single-shot agreement for every vertex, we can run it for vertices corresponding to responsive validators.
The rest of the vertices can be ordered based on causal history as previously. 
this way, in the best case, vertices corresponding to responsive validators will be ordered in 2 rounds and the rest in 3.
The worst case will become less likely.


==> sections/leaderreputation.tex <==
%Leader reputation is a property that many times overlooked in BFT literature but has a significant impact on production performance.

\subsection{Leader Reputation}
\label{sec:leaderreputation}
BFT systems are designed to tolerate Byzantine failures in order toprovide as strong as possible worst-case reliability guarantees.
However, actual Byzantine failures rarely occur in practice.
This is because validators are highly secured and have strong economic incentives to follow the protocol.
Slow or crashed leaders are a much more frequent occurrence which can significantly degrade the system performance.
In Narwhal-based BFT, if the leader of round $r$ crashes, no validator will have the anchor of round $r$ in its local view of the DAG. 
Thus, the anchor will be skipped and no vertices in the previous round can be ordered until some later point due to an anchor in a future round.

The way to deal with missing anchors is to somehow ensure that the corresponding leaders are less likely to be elected in the future.
%slow/crashed leaders that are not able to drive the protocol progress is to make sure they are less likely to be elected in the future.
A natural approach to this end is to maintain a reputation mechanism, assigning each validator a score based on the history of its recent activity. A validator that has been participating in the protocol and has been responsive would be assigned a high score. Otherwise, the validator is likely having some issues and a low score is assigned.
The idea is then to deterministically re-compute the pre-defined mapping from rounds to leaders every time the scores are updated, biasing towards leaders with higher scores. In order for validators to agree on the new mapping, they should agree on the scores, and thus on the history used to derive the scores.

Such a mechanism was previously proposed in~\cite{cohen2022aware} and implemented in the Diem Blockchain~\cite{diembft} to enhance the performance of Jolteon~\cite{jolteon}, a leader-based consensus protocol.
One important property Jolteon is that Safety is preserved even if validators disagree on the identity of the leader, while liveness is guaranteed as long as they eventually converge.
Hence, validators could re-assign the reputation scores every time a new block was committed, even though during asynchronous periods it was possible for different validators to commit the same block in different rounds.
Unfortunately, this is not the case for Narwhal-based BFT. If validators disagree on the anchor vertices, they will order the DAG differently and thus violate safety.
This makes the leader reputation problem strictly harder in Narwhal-based BFT. 

\paragraph{Solution}
\sysname constructs a protocol identical to a given Narwhal-based consensus protocol $\mathcal{P}$, but to support leader reputation anchors are selected according to a function $F$ that takes into account validators' recent activity, e.g., the number of vertices they have successfully added to the DAG.
The function $F$ should be updated as frequently as possible and aim to select validators with better reputation as leaders more often than their counterparts with lower reputation.

In \sysname, pipelining and leader reputation can be naturally combined as they both utilize the same core technique of re-interpreting the DAG after agreeing on the first ordered anchor. 
In fact, the pseudocode for \sysname appears in Algorithm~\ref{alg:leaderreputation} only differs from Algorithm~\ref{alg:pipelining} by adding line~\ref{line:updatingF2}.
The idea is that the validators simply need to compute a new mapping, starting from round $r+1$, based on the causal history of ordered anchor $A$ in round $r$ (which they are guaranteed to agree on by Property~\ref{pro:firstanchor}). Then, the validators start executing a new instance of $\mathcal{P}$ from round $r+1$ with the updated anchor selection function $F$. 

\begin{algorithm}
\caption{\sysname}
\begin{algorithmic}[1]
        \State $\emph{current\_round} \gets 0$
        \State $F: R \rightarrow A$
        \Comment{deterministic rounds to anchors mapping}
        \While{\emph{true}}
        \State execute $\mathcal{P}$, select anchors by $F$, starting from \StateX\emph{current\_round} until the first ordered (not skipped)
        \StateX anchor is determined.

        \State let $A$ be the first ordered anchor in round $r$
        \State order $A$'s causal history according to $\mathcal{P}$ 
        %\Statex \hspace{4.5mm} deterministic rule
        \State $\emph{current\_round} \gets r+1$ 
        \State update $F$ according to $A$'s causal history
        \label{line:updatingF2}
        \EndWhile
\end{algorithmic}
\label{alg:leaderreputation} 
\end{algorithm}

Our solution is protocol agnostic and can be directly applied to all Narwahl-based consensus protocols, i.e., DAG-Rider, Tusk, and Bullshark. An illustration can be found in Figure~\ref{fig:leaderreputation}.
\sysname makes no changes to the protocols but rather combines their instances, and the entire correctness argument can be derived solely from Property~\ref{pro:firstanchor}.

%The illustration can be found in Figure~\ref{fig:leaderreputation}

%The pseudocode appears in Algorithm~\ref{alg:leaderreputation}.
%At the beginning of the protocol, all validators interpret the DAG from round $0$, and the function $F$ is some pre-defined deterministic mapping. Each validator locally runs $\mathcal{P}$, using $F$ to determine the anchors, until it orders the first anchor, denoted by $A$ in round $r$.
%By the correctness of $\mathcal{P}$, as stated in Property~\ref{pro:firstanchor}, all validators agree that $A$ is the first ordered anchor.
%Consequently, each validator can re-interpret the DAG from the next round (round $r+1$) according to a new instance of the protocol $\mathcal{P}$ (or another Narwhal-based protocol) executing from scratch from round $r+1$.

%To incorporate leader reputation, the validators update the function $F$ according to the information in $A$'s causal history. 
%By completeness, all validators observe the same causal history of anchor $A$, and thus they all make identical updates to the function $F$.
%Thus, validators order $A$'s causal history and start executing a new instance of $\mathcal{P}$ from round $r+1$ with the updated anchor selection function $F$. 


\begin{figure}
    \centering
    \includegraphics[width=0.48\textwidth]{figures/leaderreputation.pdf}
    \caption{Illustration of \sysname's leader reputation integrated into Bullshark (no pipelining). 
    First, the DAG is interpreted via the Bullshark protocol and the red anchors. The anchor in round i+1, A1, is determined to be the first ordered anchor. 
    Then, based on A1's causal history, new anchors are selected for future rounds (marked in green). 
    Note that validator 4, which had an anchor according to the red selection, no longer has an anchor according to the new mapping (it was not performing well).
    Then, A1's causal history is deterministically ordered as in the original Bullshark, and a new instance of Bullshark starts at round $i+2$ based on the green anchors.}
    
    \label{fig:leaderreputation}
\end{figure}


%Correctness of the scheme still follows from Property~\ref{pro:firstanchor}.



%Each validator starts executing an instance of $\mathcal{P}$ until it determines the first non-skipped anchor (in other words, the anchor that is ordered first) according to the local deterministic ordering rule of $\mathcal{P}$ based on the validator's local view of the DAG. 
%The key is that by Property~\ref{pro:firstanchor} all validators agree on which anchor is ordered first.
%Let $A$ be this anchor in round $r$.





%Since all validators agree on the same anchor $A$, they can all start a new instance of $\mathcal{P}$ from round $r+1$. 

%In order to start a new instance of $\mathcal{P}$ in round $r+1$, validators need to agree on the mapping from rounds to leaders.

%One way is to use the same mapping as the original one but shift it to start from round $r+1$.




%As we analyze below, in the best case \sysname orders an anchor every round.  
%For Bullshark, this means anchors have 2 rounds of latency and the rest 3.


==> sections/pipelining.tex <==
\section{\sysname}

\sysname is protocol agnostic and can be directly applied to all Narwhal-based consensus protocols, i.e., DAG-Rider, Tusk, and Bullshark.
It makes no changes to the protocols but rather combines their instances in essentially a ``black-box" manner. 
The entire correctness argument can be derived solely from Property~\ref{pro:firstanchor}.

\subsection{Pipelining} 
\label{sec:pipelining}
A natural progression after the high throughput scalability of BFT consensus achieved by Narwhal is to reduce latency as much as possible.
To this end, Bullshark already halved DAG-rider's latency for ordering anchors from 4 rounds to 2 by adding an optimistic path under the partially synchronous network communication assumption.

Intuitively, it is hard to imagine latency lower than 2 rounds as in the interpretation of the DAG structure as a consensus protocol, one round is needed to "propose" the anchor, while another is needed for "voting". 
However, only anchors can be ordered in 2 rounds. 
The rest of the vertices are ordered as part of the causal history of some anchor and require a minimum latency of 3 or 4 rounds.
This is because the vertices in a "voting" round require a minimum of 3 rounds, while vertices that share a round with an anchor have to wait for at least the next anchor to be ordered, thus requiring a minimum of 4 rounds.
An illustration of the ordering latency for different vertices appears in Figure~\ref{fig:latency}.

\begin{figure}
    \centering
    \includegraphics[width=0.48\textwidth]{figures/latency.pdf}
    \caption{Illustration of the number of rounds required for each vertex in the DAG to be ordered in the best case, according to the Bullshark protocol. The number in each vertex represents its minimum latency. 
    For example, the anchor of round $i+1$ can be ordered in round $i+2$, but the other vertices in this round require at least 4 rounds to be ordered.}
    
    \label{fig:latency}
\end{figure}

Ideally, to reduce the latency of ordering vertices we would like to have an anchor in every round.
This would allow for non-anchor vertices to be ordered as a part of some anchor's causal history in each and every round, making latency and throughput of the protocol less spiky. 
%This would reduce the latency of all vertices to the minimum possible by the protocol's order rule and make the throughput less spiky. 
In Bullshark, it would become possible for every non-anchor vertex to be ordered in 3 rounds (see Figure~\ref{fig:latency}), while in DAG-Rider the latency may be reduced from 10 rounds to 7 in expectation. 

\paragraph{Solution}
Let $\mathcal{P}$ be any Narwhal-based consensus protocol.
On a high level, the core technique in \sysname is to execute $\mathcal{P}$ until it, as a consensus protocol, guarantees agreement on some part of the DAG for all validators.
%\sasha{This is not clear. I think we should link the property and talk directly about the first ordered anchor. Otherwise, what prefix?
%Also, below you say "the next round". Next after what?
%edit: moe details are given below so this flaf might be fine. But in any case I would start with "intuitively" or "on a high level" to emphasize that we are being imprecise here.}
Starting from the round following the agreed part of the DAG, all validators can switch over and start executing a new instance of $\mathcal{P}$ (or a different Narwhal-based consensus protocol, if desired) from scratch.
While the instances are not executing concurrently, this scheme effectively pipelines the ``proposing" and ``voting" rounds. As a result in \sysname, in a good case, an anchor is ordered in every round.

The pseudocode appears in Algorithm~\ref{alg:pipelining}.
In the beginning of the protocol, all validators interpret the DAG from round $0$, and the function $F$ is some pre-defined deterministic mapping from rounds to leaders.
Each validator locally runs $\mathcal{P}$, using $F$ to determine the anchors, until it orders the first anchor, denoted by $A$ in round $r$.
The key is that, by the correctness of $\mathcal{P}$ as stated in Property~\ref{pro:firstanchor}, all validators agree that $A$ is the first ordered anchor (previous anchors are skipped by all validators).
Consequently, each validator can re-interpret the DAG from the next round (round $r+1$) according to a new instance of the protocol $\mathcal{P}$ (or another Narwhal-based protocol) executing from scratch from round $r+1$.

\begin{algorithm}
\caption{Pipelining in \sysname}
\begin{algorithmic}[1]
        \State $\emph{current\_round} \gets 0$
        \State $F: R \rightarrow A$
        \Comment{deterministic rounds to anchors mapping}
        \While{\emph{true}}
        \State execute $\mathcal{P}$, select anchors by $F$, starting from \StateX\emph{current\_round} until the first ordered (not skipped)
        \StateX anchor is determined.

        \State let $A$ be the first ordered anchor in round $r$
        \State order $A$'s causal history according to $\mathcal{P}$ 
        %\Statex \hspace{4.5mm} deterministic rule
        \State $\emph{current\_round} \gets r+1$ 
        %\State update $F$ according to $A$'s causal history
        %\label{line:updatingF2}
        %\State $F(x) \gets F(x - \emph{current\_round})$
        \EndWhile
\end{algorithmic}
\label{alg:pipelining} 
\end{algorithm}



To order the DAG, much like in the original $\mathcal{P}$, the validators deterministically order $A$'s causal history, and by the Completeness property, arrive at the same total order over the same vertices.
Note that without re-interpreting the DAG according to a new instance of $\mathcal{P}$ starting from round $r+1$, the next anchor according to the previously executing instance of the protocol would appear in a strictly later round (e.g. $r+4$ for Dag-Rider and $r+2$ for Bullshark).
The above process can continue for as long as needed.
An illustration appears in Figure~\ref{fig:pipelining}.

\begin{figure}
    \centering
    \includegraphics[width=0.48\textwidth]{figures/pipelining.pdf}
    \caption{Illustration of \sysname's pipelining integrated into Bullshark.
    The vertices that are fixed to be anchors by $F$ are marked by a crown.
    The protocol starts by interpreting the DAG with anchors in rounds $1, 3$, and $5$, and Bullshark determines that the anchor in round 1, marked by a green checkmark, is the first to be ordered. 
    Then, a new instance of Bullshark starts at round 2 with the anchors marked in rounds $2$ and $4$.}
    \label{fig:pipelining}
\end{figure}

Note that in Algorithm~\ref{alg:pipelining}, function $F$ is fixed and used by each instance of protocol $\mathcal{P}$. In a true "black-box" implementation, the round numbers could be different from the perspective of the executing protocol instance (i.e. start from $0$ for each new instance). However, $F$ is fixed and always assigns the same anchor to any given round $r$ in \sysname regardless of the protocol instance used for this round. 
%\sasha{Should we add that F is fixed for presentation purposes?}
